Impact of Tool Support in Patch Construction

In this work, we investigate the practice of patch construction in the Linux kernel development, focusing on the differences between three patching processes: (1) patches crafted entirely manually to fix bugs, (2) those that are derived from warnings of bug detection tools, and (3) those that are automatically generated based on fix patterns. With this study, we provide to the research community concrete insights on the practice of patching as well as how the development community is currently embracing research and commercial patching tools to improve productivity in repair. The result of our study shows that tool-supported patches are increasingly adopted by the developer community while manually-written patches are accepted more quickly. Patch application tools enable developers to remain committed to contributing patches to the code base. Our findings also include that, in actual development processes, patches generally implement several change operations spread over the code, even for patches fixing warnings by bug detection tools. Finally, this study has shown that there is an opportunity to directly leverage the output of bug detection tools to readily generate patches that are appropriate for fixing the problem, and that are consistent with manually-written patches.

==> discussions.tex <==
\section{Discussions}

\subsection{Implications}

\tb{If automated repair, is about avoiding downtime, researchers should focus on binary fixes,
or on on-the-fly runtime recovery. Source-code repair should be aligned with developers constraints 
on code readability, style, etc.}



\subsection{Limitations \& Threats to Validity}

- Per pure conservatism, we do not consider patches which do not have a link to a bug report, including
silent bug fix patches (i.e., those patches that correct faults without mentioning them)



==> sections/api.tex <==
\subsection{API usage vs API definition fixes}
A recurrent criticism~\cite{Zhong:2015:ESR:2818754.2818864} of current automated repair approaches is that they
do not leverage API knowledge in the design of repair actions, and will thus miss
fixing API-related bugs. Yet, Zhong et al.~\cite{Zhong:2009:IRS:1747491.1747528} have shown that, 
when developing new code~\cite{Zhong:2009:MMR:1615184.1615205} or migrating existing code~\cite{Zhong:2010:MAM:1806799.1806831},
developers who lack knowledge on APIs can carelessly introduce API-related bugs. We investigate the importance of API knowledge
 in creating manual, semi-manual and automated patches. We differentiate changes that are related to the usage of API functions from
changes that deal with the definition of API functions. 

Although the Linux kernel does not provide a well-defined API nor a stable one~\cite{kroah2013linux},
it provides support for conveniently loading a module (e.g., a device driver) into a running kernel using the loadable kernel 
module facility\cite{de1999loadable}. Such a module may interact with the kernel via those kernel functions that the 
Linux kernel developers have chosen to export using the {\tt EXPORT\_SYMBOL} mechanism. We thus collect such functions which are
considered as kernel API functions~\cite{bissyande2013contributions} and check which manual, semi-manual or automated patches
touch the usage and/or definition of API functions.

Concretely, for usage of API functions, we re-build the excerpt of code before the application of patch and
parse it with {\em ctags}\footnote{\url{http://ctags.sourceforge.net/whatis.html}} which builds an index of language
objects (e.g., functions) found in the code. If among those tags an API function in our list is mentioned then we consider
the patch to be impacting the usage of an API.


We also count the number of patches in each category that change code in the definition of API functions.\tb{@Anil, How do you do it?}

\tb{Ideally what I want to show here is that API usage is mostly fixed automatically,
while API definition changes require manual effort for understanding behaviour, or with
bug finding tools}

\begin{figure}[!htb]
	\includegraphics[width=1\linewidth]{../plots/ds/DistOfApiUsagePerc}
	\caption{Distribution of Api Usage in Percentage.}
	\label{fig:distOfApiUsagePerc}
\end{figure}

